Scalar leptoquarks at the LHC and flavour anomalies: a comparison of pair-production modes at NLO-QCD

We analyse scalar leptoquark pair production at the LHC with predictions including $t$-channel lepton exchange contributions up to next-to-leading order (NLO) in QCD. In particular, we calculate NLO-QCD predictions for off-diagonal production channels, {\it i.e.}\ channels that involve two different leptoquark eigenstates and are driven solely by diagrams involving Standard Model leptons in the $t$-channel at leading order, as opposed to diagonal channels where a pair of the same leptoquark eigenstate is produced. We find that reliable theoretical predictions for both channels require NLO accuracy. The relative importance of the off-diagonal modes depends strongly on the considered scenario. In a generic model involving $R_2$ and $S_3$ leptoquarks, at large values of the Yukawa couplings off-diagonal contributions initiated by valence quarks can be up to an order of magnitude higher than the diagonal production. However, we also find that in phenomenologically viable scenarios addressing the flavour anomalies off-diagonal production is generally negligible, with a few exceptions of 10\%--30\% of the total rate depending on the treatment of the charm density in the proton.

==> Sections/Introduction_2022-10-14.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}
\label{sec:intro}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Scalar leptoquarks are scalar bosons beyond the Standard Model which carry both lepton and baryon numbers, and therefore couple simultaneously to leptons and quarks via a Yukawa-type interaction. Originally proposed in models of Grand Unification \cite{Pati:1973uk,Pati:1974yy,Georgi:1974sy,Fritzsch:1974nn,Senjanovic:1982ex,Frampton:1989fu,Murayama:1991ah}, they appear in many extensions to the Standard Model, \eg~in superstring models \cite{Hewett:1988xc}, $R$-parity violating supersymmetric scenarios \cite{Farrar:1978xj,Barbier:2004ez}, composite models \cite{Dimopoulos:1979es,Eichten:1979ah,Farhi:1980xs,Schrempp:1984nj,Lane:1991qh}, neutrino mass models~\cite{Dorsner:2005fq,Babu:2010vp,Babu:2019mfe,Bigaran:2019bqv,Julio:2022ton,Julio:2022bue}, or as mediators in simplified models of dark matter \cite{Baker:2015qna,Choi:2018stw,Guadagnoli:2020tlx,Arcadi:2021cwg,Belanger:2021smw,Baker:2021llj}. Scalar leptoquarks may also offer an explanation \cite{Hiller:2014yaa,ColuccioLeskow:2016dox,Crivellin:2017zlb,Hiller:2018wbv,Crivellin:2020tsz,Angelescu:2021lln,Nomura:2021oeu,Marzocca:2021azj,FileviezPerez:2021lkq,Murgui:2021bdy,Singirala:2021gok,Crivellin:2022mff} to the anomalies appearing in $B$-physics observables~\cite{BaBar:2012obs,Belle:2019oag,BELLE:2019xld,Belle:2019rba,LHCb:2017avl,LHCb:2017smo,LHCb:2019hip,LHCb:2021trn}, as well as to the discrepancy between theoretical predictions \cite{Aoyama:2020ynm} and experimental measurements \cite{Muong-2:2006rrc,Muong-2:2021ojo} related to the anomalous magnetic moment of the muon. In this context, most interesting scenarios feature large Yukawa couplings between leptons, quarks, and leptoquarks.

The ATLAS and CMS collaborations at the Large Hadron Collider (LHC) have so far measured no signals hinting at the existence of scalar leptoquarks, thus pushing {\color{red}the mass limits up to around 1.0--1.8\,TeV~\cite{ATLAS:2019qpq,ATLAS:2020dsf,ATLAS:2020dsk,ATLAS:2021oiz,ATLAS:2021yij,ATLAS:2021jyv,ATLAS:2022ors,ATLAS:2022fho,ATLAS:2022wgt,CMS:2018txo,CMS:2018lab,CMS:2018iye,CMS:2018ncu,CMS:2020wzx,CMS:2021far,CMS:2022nty}. The precise value of the bounds depend on the considered leptoquark model (in particular on the texture in the flavour space of the leptoquark Yukawa couplings), as well as on the production mechanism targeted by the different searches.} The most stringent limits originate from LHC direct searches for the pair production of scalar leptoquarks, assuming that the Yukawa couplings are small so that the production is driven purely by QCD interactions{\color{red}. Leptoquark masses are hence constrained to be larger than 1.8~TeV~\cite{ATLAS:2020dsk,CMS:2018ncu,CMS:2021far}, 1.7~TeV~\cite{ATLAS:2020dsk,CMS:2018lab} and 1.4~TeV~\cite{ATLAS:2019qpq,ATLAS:2020dsf,ATLAS:2021oiz,ATLAS:2021yij,ATLAS:2021jyv,CMS:2018iye,CMS:2020wzx} for leptoquarks coupling to first-generation, second-generation and third-generation fermions respectively. Moreover, mixed leptoquark decay patterns into leptons and quarks of different generations have been studied, which has led to mass limits of about 1.7--2.0~TeV for both the electron and muon channels~\cite{ATLAS:2020dsk,ATLAS:2022ors,ATLAS:2022wgt}.} The assumption {\color{red}of a small Yukawa coupling is however} clearly at odds with possible explanations of lepton flavour anomalies. Consequently, Yukawa coupling-induced contributions ought to be included in studies of leptoquark production at the LHC. {\color{red}Such a large Yukawa coupling assumption also renders other leptoquark production modes relevant, and bounds of 1.4~TeV~\cite{ATLAS:2022fho,CMS:2018txo,CMS:2020wzx,CMS:2022nty} have correspondingly been obtained for the third-generation leptoquark case. These mass limits can nevertheless be weakened or even evaded by reducing the size of the leptoquark Yukawa couplings.}

From the theoretical side, calculations for cross sections of scalar leptoquark pair production are available at the next-to-leading order (NLO) in the strong coupling constant $\alphas$ already for some time \cite{Kramer:1997hh,Kramer:2004df}. More recently these fixed-order calculations have been matched with parton showers~\cite{Dorsner:2018ynv,Mandal:2015lca}, and with soft-gluon resummation up to next-to-next-to-leading logarithmic accuracy \cite{Borschensky:2020hot, Borschensky:2021hbo,Borschensky:2021jyk}. In the latter works, in addition to the pure-QCD contribution, also so-called $t$-channel contributions (\ie~diagrams with a $t$-channel lepton exchange that are proportional to the leptoquark Yukawa couplings) have been taken into account. It has been shown that for phenomenologically relevant parameter points, these additional terms can be sizeable and can interplay in an intricate way with soft-gluon corrections. Furthermore, the expected production rates turns out to depend strongly on the chosen leptoquark model and benchmark scenario, as well as on the set of parton distribution functions (PDF) used for the calculations. All these effects need thus to be considered for the best exploitation of scalar leptoquark searches.

Besides pair production of scalar leptoquarks, other relevant processes for leptoquark searches at hadron colliders include their single production in association with a lepton~\cite{Hiller:2018wbv,Alves:2002tj,Dorsner:2014axa,Hammett:2015sea,Mandal:2015vfa,Haisch:2022afh} {\color{red}(for which predictions are known at NLO in QCD~\cite{Dorsner:2018ynv,Haisch:2022afh})}, Drell-Yan di-lepton production with leptoquarks appearing as virtual particles~\cite{Faroughy:2016osc,Raj:2016aky,Greljo:2017vvb,Bansal:2018eha,Schmaltz:2018nls,Fuentes-Martin:2020lea,Haisch:2022lkt}, and resonant leptoquark production through quark-lepton initial states~\cite{Ohnemus:1994xf,Eboli:1997fb,Buonocore:2020erb,Greljo:2020tgv,Buonocore:2022msy}. Recently, a novel channel related to the pair production of scalar leptoquarks has been introduced~\cite{Dorsner:2021chv}. In certain scenarios with at least two leptoquark eigenstates, there exists the possibility to produce a `diagonal' pair of leptoquarks of the same eigenstate, or to `off-diagonally' produce two different leptoquark states. In contrast to the diagonal production, the off-diagonal channel is, at tree level, purely driven by the strength of the leptoquark Yukawa couplings and independent of the strong coupling constant. In addition, the quark-quark channel opens up, with quarks of possibly unequal flavours. This is particularly suited for LHC studies as one can expect large cross sections if two valence quarks are involved. For instance, it has been shown at leading order (LO) in~\cite{Dorsner:2021chv} that for a one-flavour new physics realisation based on a model including both $S_1$ and $R_2$ leptoquarks, the {\it total} pair production rates  can be enhanced strongly relative to the expectation from pure QCD production, and this even for moderate leptoquark Yukawa couplings. In addition, the off-diagonal production channels have the potential to outweigh the importance of other Yukawa-coupling-dependent search channels, especially for moderate to large Yukawa couplings.

In the present work, we investigate the relevance of the off-diagonal production mechanism in more detail, in particular in the context of models relevant for explaining flavour anomalies. 
Given the impact of higher-order QCD effects on the predictions for scalar leptoquark pair-production reported in~\cite{Borschensky:2020hot, Borschensky:2021hbo,Borschensky:2021jyk}, and generally their relevance for the production of heavy coloured particles in hadronic channels, we increase the precision of the off-diagonal production mechanism of scalar leptoquarks by calculating the associated NLO-QCD corrections. We also compare the off-diagonal production rates with diagonal production through both QCD and  Yukawa coupling-induced $t$-channel mechanisms. The computations are included in our framework of scalar leptoquark pair production for various leptoquark models \cite{Borschensky:2020hot,Borschensky:2021hbo,Borschensky:2021jyk} with the \mgamc{}~\cite{Alwall:2014hca} and \pwb~\cite{Nason:2004rx,Frixione:2007vw,Alioli:2010xd} software. In addition, we comprehensively study the impact of the Yukawa-coupling-driven contributions on inclusive rates for phenomenologically viable leptoquark models that offer a solution to the flavour anomalies.

The structure of this paper is as follows. In section~\ref{sec:models}, we discuss our theoretical setup and the specific benchmark leptoquark scenarios that we study, followed by a brief review of leptoquark pair production at fixed order. We then introduce some computational details in section~\ref{sec:results}, and next analyse  the numerical impact of the off-diagonal production modes on total rates. In this context, we consider a general scenario including $R_2$ and $S_3$ leptoquarks coupling to quarks of the first and second generation. An application of our calculations to phenomenologically viable benchmark scenarios is subsequently presented in section~\ref{sec:BSs}, where we also highlight the role of the charm PDF on production rates. At last, we conclude in section~\ref{ref:conclusions}.

